Arnold conjecture over integers

For any closed symplectic manifold, we show that the number of 1-periodic orbits of a nondegenerate Hamiltonian thereon is bounded from below by a version of total Betti number over Z of the ambient space taking account of the total Betti number over Q and torsions of all characteristic. The proof is based on constructing a Hamiltonian Floer theory over the Novikov ring with integer coefficients, which generalizes our earlier work for constructing integer-valued Gromov-Witten type invariants. In the course of the construction, we build a Hamiltonian Floer flow category with compatible smooth global Kuranishi charts. This generalizes a recent work of Abouzaid-McLean-Smith, which might be of independent interest.

==> Old.tex <==

\section{Old approach}

\subsection{Equivariant smoothing theory}

\subsubsection{Finite group actions on topological manifolds}

We first review basic facts and subtlety about group actions on topological manifolds. Let $M$ be an $n$-dimensional topological manifold. That is, a second countable Hausdorff topological space which is locally homeomorphic to ${\mb R}^n$. Let $G$ be a finite group. A continuous $G$-action on a topological manifold $M$ is called {\bf locally linear} if for each $x \in M$ whose stabilizer is $G_x \subseteq G$, there exist a representation $V_x$ of $G_x$, a $G_x$-invariant neighborhood $U_x\subseteq M$, and a $G_x$-equivariant continuous map $U_x \to V_x$ which is a homeomorphism onto an open neighborhood of the origin. 

A subtlety about locally linear actions is that the local linear model is not unique. We need to specify 
\begin{defn}
A {\bf linearized topological $G$-manifold} consists of a topological manifold with a locally linear $G$-action together with a choice of a finite-dimensional real $G_x$-representation $V_x$ for all $x \in M$ satisfying the following condition. For each $x$, there exists a $G_x$-equivariant homeomorphism $\phi_x: D(V_x) \to M$ from an open ball $D(V_x) \subseteq V_x$ onto an open neighborhood of $x$ sending the origin to $x$. Moreover, for each $y \in {\rm Im} \phi_x$, the map $\phi_x$ induces an inclusion $G_y \hookrightarrow G_x$ and then $V_y$ is isomorphic to $V_x$ viewed as a $G_y$-representation. (We also need to fix the isotopy classes of such $\phi_x$).
\end{defn}

An important tool is the equivariant version of the isotopy extension theorem. 

\begin{thm}(Equivariant isotopy extension)\cite[Theorem 4.4]{Lashof_Rothenberg} Suppose $M$ is a locally linear topological $G$-manifold, $K \subseteq M$ is a $G$-invariant compact subset, and $V \subseteq M$ is a $G$-invariant open neighborhood of $K$. Let $f_t: V \to M$, $t \in [0, 1]$ be a continuous family of open $G$-embeddings with $f_0$ being the inclusion of $V$. Then there exists a continuous family $F_t: M \to M$ of $G$-equivariant homeomorphisms such that $F_t|_K = f_t|_K$ and $F_t$ is the identity map outside an open neighborhood of $K$. 
\end{thm}






\subsubsection{Microbundles}

Smoothing theory is closely related to the theory of microbundles invented by Milnor \cite{Milnor_micro_1}. 

\begin{defn}
Let $B$ be a topological space. 
\begin{enumerate}
    \item A {\bf microbundle} over $B$ is a diagram
\beqn
\mu =( \xymatrix{B \ar[r]^i & E \ar[r]^p & B} )
\eeqn
of topological spaces and continuous maps satisfying the following conditions:
\begin{enumerate}
    \item $p \circ i = {\rm id}_B$;
    
    \item For each $b \in B$ there exist an open neighborhood $U$ of $b$, an open neighborhood $V$ of $i(b)$, a homeomorphism $f: V \cong U \times {\mb R}^n$ such that $i(U) \subseteq V$, $\pi(V) \subseteq U$, and the following diagram commutes.
    \beqn
    \xymatrix{  & V \ar[dd]^f \ar[rd]^p & \\
               U \ar[ru]^i \ar[rd]^0 & & U \\
               &  U \times {\mb R}^n \ar[ru]^{p_1} & }
    \eeqn
    \end{enumerate}
    
    \item A morphism $\phi$ from a microbundle $\mu =(\xymatrix{B \ar[r]^{i} & E \ar[r]^{p} & B})$ over $B$ to a second microbundle $\mu' = (\xymatrix{B \ar[r]^{i'} & E' \ar[r]^{p'} & B})$ over the same base is the germ of continuous maps $\phi: U \to E'$ defined over a neighborhood $U$ of $i(B)$ which commutes with $i, i'$ and $p, p'$. The morphism $\phi$ is called an {\bf isomorphism} if $\phi$ is a homeomorphism onto an open neighborhood of $i'(B)$.
    \end{enumerate}
    \end{defn}

Microbundles are generalizations of vector bundles. If $E \to B$ is a vector bundle, then the diagram 
\beqn
\mu_E = ( \xymatrix{ B \ar[r]^s & E \ar[r]^\pi & B})
\eeqn
consisting of the zero section and the bundle projection is obviously a microbundle. 

An important fact regarding microbundles is the Kister--Mazur theorem. An ${\mb R}^n$-bundle over $B$ is a fibre bundle $E \to B$ with fibres being ${\mb R}^n$ and the structure group being ${\rm Top}_n$, the group of homeomorphisms of ${\mb R}^n$ which fix the origin. Then each ${\mb R}^n$-bundle has a zero section and hence induces a microbundle. The Kister--Mazur theorem (\cite{Kister_1964}\cite{Mazur_1964}) says that microbundles are essentially ${\mb R}^n$-bundles. More precisely one has the following theorem.
\begin{thm}(Kister--Mazur Theorem) 
Let $B$ be a topological manifold.\footnote{In fact the theorem holds for ``sufficiently nice'' spaces.} Then for each microbundle $\mu$ over $B$, there exists an ${\mb R}^n$-bundle $E \to B$ with an isomorphism of microbundles $\phi: \mu_E \to \mu$.
\end{thm}

\begin{example}
Let $M$ be a topological manifold. Its {\bf tangent microbundle} is the diagram 
\beqn
\tau M = ( \xymatrix{M \ar[r]^-i & M \times M \ar[r]^-{p_1} & M } )
\eeqn
where $i: M \to M\times M$ is diagonal embedding and $p_1: M \times M \to M$ is the projection onto the first factor. By abuse of notation, any microbundle which is equivalent to the above $\tau M$ is also called the tangent microbundle of $M$. 
\end{example}

\begin{example}
Let $M$ be a topological submanifold and $S \subset M$ be a topological submanifold. That is, $S$ with the subspace topology is a topological manifold. A {\bf normal microbundle} to the embedding $S \hookrightarrow M$ is a microbundle $\mu = ( \xymatrix{ S \ar[r]^i & E \ar[r]^p & S} )$ where $E \subset M$ is an open neighborhood of $S$ and $i: S \to E$ is the inclusion. Not all topological submanifolds admit normal microbundles and a necessary (but not sufficient) condition is that $S$ being a locally flat submanifold. 
\end{example}




\subsubsection{Classifying spaces}

Let $A$ be a topological group and $G$ be a finite group. Let $B$ be a $G$-space. A principal $G$-$A$ bundle over $B$ is a principal $A$-bundle $\pi: P \to B$ which has a left $G$-action such that $\pi$ is equivariant. 

\begin{thm}(\cite{SJHu_thesis}, cf.\cite[Theorem 1.7]{Lashof_Rothenberg})
There exists a universal $G$-$A$ bundle.
\end{thm}

Now consider the topological group ${\rm Top}_n$ which is the group of homeomorphisms of ${\mb R}^n$ which fix the origin, equipped with the compact-open topology. The orthogonal group $O_n\subset {\rm Top}_n$ is a subgroup. Let the classifying spaces of $G$-${\rm Top}_n$ bundles and $G$-$O_n$ bundles be $B{\rm Top}_n(G)$ and $BO_n(G)$ respectively. They classify $G$-equivariant ${\mb R}^n$-bundles and $G$-equivariant (real) vector bundles. 

Now suppose $M$ is a topological $G$-manifold. By the $G$-Kister theorem (see \cite[Theorem 2.7]{Lashof_Rothenberg}), the microbundle $\tau M$ contains an $G$-equivariant ${\mb R}^n$-bundle whose isomorphism class is canonically associated to $\tau M$. Therefore, there is a classifying map (well-defined up to homotopy)
\beqn
\tau: M \to B{\rm Top}_n(G).
\eeqn



\subsubsection{$G$-smoothing theory}

We discuss the equivariant smoothing theory (for finite groups) developed by Lashof--Rothenberg \cite{Lashof_Rothenberg}.








A {\bf smoothing} of $M$ is a pair $({\bm M}, \phi)$ where ${\bm M}$ is a smooth manifold and $\phi: {\bm M}\to M$ is a homeomorphism. Two smoothings $({\bm M}_i, \phi_i)$, $i = 1, 2$, are {\bf isomorphic} if the composition 
\beqn
\phi_2^{-1} \circ \phi_1: {\bm M}_1 \to {\bm M}_2
\eeqn
is a diffeomorphism. Two such smoothings are called {\bf isotopic} if $\phi_1$ is isotopic to another homeomorphism $\phi_1': {\bm M}_1 \to M$ such that $({\bm M}_1, \phi_1')$ and $({\bm M}_2, \phi_2)$ are isomorphic. 

One has similar notions in the equivariant case. A {\bf $G$-smoothing} of a $G$-manifold $M$ is a smoothing $({\bm M}, \phi)$ such that ${\bm M}$ is a smooth $G$-manifold and $\phi$ is $G$-equivariant. 


\begin{thm}\cite[Theorem 6.9]{Lashof_Rothenberg} Let $M$ be a locally smooth $G$-manifold without boundary such that for each subgroup $H \subseteq G$, the fixed point set $M^H \subset M$ contains no 4-dimensional component. Then the isotopy classes of $G$-smoothings of $M$ are in one-to-one correspondence with the isotopy classes of $G$-vector bundle reductions of $\tau M$.
\end{thm}







\subsubsection{A theorem about tubular neighborhoods}

We first specify our notion of tubular neighborhoods, which is stronger than normal microbundles. 

\begin{defn}(Topological tubular neighborhood)
Let $M$ be a topological manifold and let $S\subset M$ be a topological submanifold. 
\begin{enumerate}
    \item A {\bf tubular neighborhood} of $S$ is $(D, \rho)$ where $D \to S$ is an (open) disk bundle (contained in a vector bundle $E \to S$) and $\rho:D \to M$ is a homeomorphism onto an open neighborhood of $S$ such that $\rho|_S$ is the identity map of $S$.
    
    \item Two tubular neighborhoods $(D_1, \rho_1)$ and $(D_2, \rho_2)$ are called {\bf isotopic} if there is an isotopy $\phi_t: M \to M$ such that $\phi_0 = {\rm Id}_M$, $\phi_t|_S = {\rm Id}_S$, and $\rho_1 = \phi_1 \circ \rho_2$.
    
    \item Suppose $G$ is a finite group acting on $M$ and $S$ is $G$-invariant. A $G$-tubular neighborhood is a tubular neighborhood $(D, \rho)$ where $D\subset E$ is a $G$-invariant disk bundle contained in an equivariant vector bundle $E \to S$ and $\rho$ is equivariant. Two $G$-tubular neighborhoods are {\bf $G$-isotopic} if they are isotopic via a path of $G$-equivariant maps.
    \end{enumerate}
    
\end{defn}

We know that for a smooth submanifold, there is essentially one tubular neighborhood modulo isotopy and orientation. It is not clear to us if uniqueness is true for topological tubular neighborhoods. However, we prove such a result for a special case. 

\begin{prop}
Let $G$ be a finite group and let $M$ be a smooth $G$-manifold. Let $M^G\subset M$ be the $G$-fixed point set. Then any $G$-equivariant tubular neighborhood is isotopic to a smooth $G$-equivariant tubular neighborhood.
\end{prop}

\begin{proof}
Consider the normal bundle $N(M^G) \to M^G$. We know $G$-vector bundles are locally trivial. Hence we can choose a countable open cover $\{ U_\alpha^G\ |\alpha=1, \ldots \}$ of $M^G$ such that $NM^G|_{U_\alpha^G}$ is (smoothly) trivial. 
\end{proof}

\begin{lemma}
Let $E, F\to B$ be two smooth vector bundles and $\phi: E \to F$ be a continuous isomorphism. Then $\phi$ is isotopic via bundle maps to a smooth isomorphism.
\end{lemma}




\subsection{Manifold with corners}

Let $(P, \leq)$ be a finite partially ordered set containing a unique maximal element $*$. Typically elements of $P$ describe possible types of breakings of a Floer trajectory between two fixed critical points. 

\begin{defn}
\begin{enumerate}
    \item A {\bf topological $P$-manifold with corners} is a topological manifold with boundary $M$ equipped with a decomposition 
\beqn
M = \bigsqcup_{\alpha \in P} M_\alpha
\eeqn
satisfying 
\begin{enumerate}
    \item The decomposition is an abstract stratification, meaning: a) each $M_\alpha$ is locally closed, and b) $M_\alpha \cap \ov{M_\beta} \neq \emptyset \Longrightarrow M_\alpha \subseteq \ov{M_\beta} \Longleftrightarrow \alpha \leq \beta$.

    \item $M_{\alpha_*} = {\rm Int} M$. Moreover, for each $\alpha \in P$, $\ov{M_\alpha}$ is a topological manifold with boundary of dimension $n_\alpha$ and 
    \begin{align*}
        &\ M_\alpha = {\rm Int} \ov{M_\alpha},\ &\ \partial \ov{M_\alpha} = \bigsqcup_{\beta < \alpha} M_\beta
        \end{align*}
    
    \item 
    
\end{enumerate}

\item Let $M$ be a topological $P$-manifold. Given $x \in M_\alpha$, a $P$-admissible chart around $x$ is a homeomorphism
\beqn
\varphi_x: U_x \to {\mb R}^{n_\alpha} \times [0, +\infty)^{n - n_\alpha}.
\eeqn

\item Let $G$ be a group. A $G$-action on $M$ is called ... if $G$ preserves the stratification, and... 
\end{enumerate}

\end{defn}

If $M$ has a locally linear $G$-action, then for each subgroup $H \subset G$, the fixed point set $M^H \subset M$ is also a topological $P$-manifold with corners with 
\beqn
(M^H)_\alpha = (M_\alpha)^H.
\eeqn

\begin{defn}
A {\bf disk bundle neighborhood} of $M^H$ is a pair $(D, \varphi)$ where $D$ is the open unit disk bundle of an $H$-equivariant vector bundle $E \to M^H$ and $\varphi: D \to M$ is a homeomorphism onto an open neighborhood of $M^H$. 
\end{defn}





\begin{prop}
Let $M$ be a topological $P$-manifold with corners with a locally linear $G$-action. Let $K \subset M^G$ be a compact subset and $C \subset M^G$ be an open neighborhood of $K$. Suppose $(D, \phi)$ is a disk bundle neighborhood of $C$ inside $M$. Then there exist a disk bundle neighborhood $(\tilde D, \tilde\phi)$ of $M^G$, a disk bundle isomorphism $\tau: D \to \tilde D$ over a neighborhood of $K$, such that 
\beqn
\tilde \phi \circ \tau = \phi. 
\eeqn
\end{prop}

\begin{proof}
We use an inductive construction based on Lemma \ref{lemma24}. Give an absolute order to elements of $P$ as $\alpha_1, \ldots, \alpha_N$ such that
\beqn
\alpha_i \leq \alpha_j \Longrightarrow i \leq j.
\eeqn
Suppose we have constructed a ......

\end{proof}



\begin{lemma}\label{lemma24}
Let $M$ be a topological manifold with a locally linear $G$-action and let $K^G \subset M^G$ be a compact subset. Let $C^G \subset K^G$ be a closed subset and $V^G \subset M^G$ be an open neighborhood of $C^G$. Suppose $(D, \phi)$ is a disk bundle neighborhood of $C^G$ inside $M$. Then there exist a disk bundle neighborhood $(\tilde D, \tilde \phi)$ of a neighborhood of $K^G$ inside $M^G$...
\end{lemma}

\subsubsection{Proof of Lemma \ref{lemma24}}



\begin{lemma}
Let $B$ be a smooth manifold with ${\rm dim} B \geq 5$. Let $V$ be a finite-dimension representation of $G$ which does not contain a trivial $G$-summand. Let $D(V)\subset V$ be an invariant open ball centered at the origin. Suppose
\beqn
\phi: B \times D(V) \to B \times V
\eeqn
is a continuous $G$-equivariant open embedding whose restriction to $B\times \{0\}$ is the identity map onto $B \times \{0\}$. Then $\phi$ is isotopic (relative to $B$) to a smooth open embedding.
\end{lemma}

\begin{proof}
Therefore, the open subset $\phi(B \times D(V)) \subset B \times V$ has two $G$-smoothings, one as an open subset of $B \times V$ and one induced by $\phi$. We will prove that these two smoothings are isotopic. Indeed, one has the following diagram.
\beqn
\xymatrix{ \phi (B \times D(V)) \ar[r]^\tau   \ar@/^2.0pc/[rr] & B{\rm Top}_n(G) & BO_n(G) \ar[l] \\
           B \ar@{^{(}->}[u] \ar[r]^{\uds\tau} \ar@/_2.0pc/[rr] & B{\rm Top}_{n-k}(G) \ar[u]^{\oplus V} & BO_{n-k}(G) \ar[u]^{\oplus V} \ar[l] }
\eeqn
Here $\tau$ and $\uds\tau$ are the classifying maps of the tangent microbundles. The top curved arrow is the classifying map induced from the smoothing $\phi$ and the bottom curved arrow is the classifying map induced from the fixed smooth structure on $B$.

We claim that the above diagram commutes up to homotopy. Indeed, the square on left open depends on the topological structures; the square on the right commutes because of .....

As $B$ is $G$-homotopy equivalent to $B \times D(V)$, one has the identification
\beqn
[B, BO_n (G)]^G \cong [B \times D(V), BO_n(G)]^G
\eeqn
where $[\cdot, \cdot]^G$ is the set of homotopy classes of $G$-equivariant maps. 

The condition that ${\rm dim} B \geq 5$ implies that for any subgroup $H \subseteq G$, the dimension of the fixed point set $B \times V^H$ is not equal to 4. Then one can apply Lashof--Rothenberg's equivariant smoothing theorem. It follow that the smoothing $\phi$ is $G$-isotopic to the standard smoothing. More precisely, there exists a continuous family of equivariant open embeddings 
\beqn
\phi_t: B \times D(V) \to B\times V
\eeqn
such that $\phi_0 = \phi$ and $\phi_1$ is smooth. As $\phi_t$ is $G$-equivariant, it preserves $B$. Let $\rho_t: B \to B$ be the restriction of $\phi_t$ and denote by $\tilde \rho_t: B\times D(V) \to B\times D(V)$ the pullback of $\rho_t$. Then define 
\beqn
\tilde \phi_t = \phi_t \circ \tilde \rho_t^{-1}: B \times D(V) \to B\times V.
\eeqn
Notice that $\tilde \phi_t$ is $G$-equivariant, fixes $B$ pointwise, and is a family of open embeddings. Moreover, $\tilde \phi_0 = \phi$ and $\tilde \phi_1$ is smooth. 
\end{proof}


Local to global.

\begin{proof}
By compactness, one can choose an open cover $\{ V_\alpha\}_{\alpha \in A}$ of $K^G$ satisfying the following condition.
\begin{enumerate}
    \item For each $\alpha$, $V_\alpha \cap C^G \neq \emptyset$ implies that $V_\alpha \subset U^G$. Moreover, in this case $E|_{V_\alpha}$ is equivariantly trivial.
    
    \item For each $\alpha$, there exists a local ... 
\end{enumerate}

One can choose a finite refinement $\{ U_\beta\}_{\beta \in B}$ of $\{V_\alpha\}_{\alpha \in A}$, meaning a map $f: B \to A$ such that $U_\beta \subset V_{f(\beta)}$, satisfying the following condition. 



Define 
\beqn
U_n^G = K^G \cup \bigcup_{1 \leq i \leq n} U_{\beta_i}
\eeqn
Now we prove inductively the following statement: for each $n\geq 0$, there is a $G$-equivariant vector bundle $E_n \to U_n^G$ (of type $V$) and a disk bundle neighborhood $\phi_n: D(E_n) \to M$ which coincides with ....... Moreover, for each $\beta\in B$, the bundle $E|_{U_\beta \cap U_n^G}$ is equivariantly trivial. The $n = 0$ case is automatic. Suppose we have constructed $E_{n-1}$ and $\phi_{n-1}$ satisfying the induction hypothesis. Denote $f(\beta_n) = \alpha_n$. Then by the induction hypothesis, the restriction $E_{n-1}|_{U_{\beta_n} \cap U_{n-1}^G}$ is trivial. Then 

\end{proof}




\subsubsection{Topological transversality to Whitney stratified sets}

Let $M$ be a smooth manifold and $S \subseteq M$ be a subset. A {\bf Whitney stratification} is a decomposition 
\beqn
S = \bigsqcup_{\alpha \in A} S_\alpha
\eeqn
of $S$ into locally closed subsets satisfying the following conditions. 
\begin{enumerate}
    \item The decomposition is locally finite and satisfies the axiom of frontier, namely, $S_\alpha \cap \ov{S_\beta} \Longrightarrow S_\alpha \subseteq \ov{S_\beta}$. This induces a partial order relation on the index set $A$: $\alpha\leq \beta$ if and only if $S_\alpha \subseteq \ov{S_\beta}$.
    
    \item Each $S_\alpha$ is a smooth submanifold of $M$.
    
    \item For $\alpha < \beta$, the pair $(S_\alpha, S_\beta)$ satisfies Whitney's condition (b). 
\end{enumerate}

A classical result 


Our construction requires a notion of transversality to a Whitney stratified set for continuous maps. The classical notion of topological transversality to a topological submanifold depends on the choice of a normal microbundle. 

\begin{defn}
Let $M$ be a topological manifold of dimension $n$. A continuous map $f: M \to {\mb R}^k$ is said to be transverse to $0\in {\mb R}^k$ if the following conditions hold.
\begin{enumerate}
    \item $f^{-1}(0) \subset M$ is a locally flat topological submanifold.
    
    \item There is a normal microbundle $\xi$ of $f^{-1}(0)$ such that the restriction of $f$ to each fibre of $\xi$ is a homeomorphism onto an open neighborhood of $0\in {\mb R}^k$.
    \end{enumerate}
\end{defn}

\begin{thm}[Topological Transversality]\cite{Kirby_Siebenmann}\cite{Quinn}\cite{Quinn_1982}

\end{thm}




Because the target manifold is smooth and the Whitney stratified subset is essentially smooth, we introduce a stronger notion of transversality for continuous maps which depends on the choice of a Riemannian metric. Let $M$ be a smooth manifold and $S \subseteq M$ be a Whitney stratified set. Choose a Riemannian metric $g$ on $M$ and let $N_\alpha \to S_\alpha$ to be the normal bundle to $S_\alpha$ (defined as the orthogonal complement of $TS_\alpha \subset TM|_{S_\alpha}$. Then the exponential map in the normal direction defines a system of tubular neighborhoods
\beqn
\phi_\alpha: D(N_\alpha) \to M
\eeqn
where $D(N_\alpha) \subset N_\alpha$ is an open disk bundle (with respect to some modified smooth bundle metric). We say that the collection $\{(D(N_\alpha), \phi_\alpha\}_{\alpha \in A}$ the system of tubular neighborhoods induced from the metric $g$. 

\begin{defn}
Let $S$ be equipped with a system of smooth tubular neighborhoods. Let $N$ be a topological manifold and $f: N \to M$ be a continuous map. We say that $f$ is transverse to $S$ at $x \in N$ if either $f(x) \notin S$ or the following conditions holds. Suppose $y = f(x)\in S_\alpha$. Choose a small neighborhood $V_y \subseteq S_\alpha$ overwhich $D_\alpha$ admits a smooth trivialization $\psi_y: D_\alpha|_{V_y} \cong V_y \times {\mb R}^{k_\alpha}$. Then for a small neighborhood $U_x \subseteq N$ of $x$ satisfying $f(U_x) \subset \phi_\alpha(D_\alpha|_{V_y})$, the map 
\beqn
{\rm proj}_2 \circ \psi_y^{-1} \circ \phi_\alpha^{-1} \circ f: U_x \to {\mb R}^{k_\alpha}
\eeqn
is transverse to the origin. 
\end{defn}
It is easy to see that this notion of transversality does not depends on the choice of local trivializations of $D_\alpha$. Moreover, if $N$ is a smooth manifold, $f$ is a smooth map and is transverse to $S$ in the smooth sense, then $f$ is also transverse in the topological system with respect to any choice of system of smooth tubular neighborhoods. 

An important fact about Whitney stratifications is that transverse points form an open set (see XXXX). We need to prove the similar result in the topological category.

\begin{prop}
Suppose $S \subseteq M$ is a closed Whitney stratified set equipped with a system of smooth tubular neighborhoods. Let $N$ be a topological manifold and $f: N \to M$ be a continuous map. Then the subset of points in $N$ at which $f$ is transverse to $S$ is open.
\end{prop}

\begin{proof}
Suppose $f(x) \in S_\alpha$. 
\end{proof}











\newpage



